A robust class of languages of 2-nested words

Regular nested word languages (a.k.a. visibly pushdown languages) strictly extend regular word languages, while preserving their main closure and decidability properties. Previous works have shown that considering languages of 2-nested words, i.e. words enriched with two matchings (a.k.a. 2-visibly pushdown languages), is not as successful: the corresponding model of automata is not closed under determinization. In this work, inspired by homomorphic representations of indexed languages, we identify a subclass of 2-nested words, which we call 2-wave words. This class strictly extends the class of nested words, while preserving its main properties. More precisely, we prove closure under determinization of the corresponding automaton model, we provide a logical characterization of the recognized languages, and show that the corresponding graphs have bounded treewidth. As a consequence, we derive important closure and decidability properties. Last, we show that the word projections of the languages we define belong to the class of linear indexed languages.

==> app-nw.tex <==
% !TEX root =  main.tex

%% Appendix : Nested words

\section{Nested Words}

\paragraph*{Grammar}

We recall the grammar describing the set of nested words.
In this definition, to ease the reading, we do not explicitly
write the matching, and instead rely on the classical presentation based
on visibly pushdown languages.

$$
\mathsf{NW} \ni w ::= i\mid \epsilon \mid w_1w_2 \mid cwr \qquad\textup{where }
i,c,r\in \Sigma
$$
and where $i$ corresponds to an internal position (no matching), and
$M(c,r)$ holds, \emph{i.e.} positions corresponding
to $c$ and $r$ respectively are in relation w.r.t. matching $M$.

More formally, the matching relation of $w_1w_2$
is defined as the union of those of $w_1$ and $w_2$ (up to shifting the interval).
That of $cwr$ is obtained by extending that of $w$
by adding a matching between positions corresponding to
$c$ and $r$. As usual, we denote by $L(\mathsf{NW})$
the language generated from $\mathsf{NW}$ using this grammar.


\paragraph*{Nested Word Automata}

%\marginpar{PA: je n'ai pas mis à jour}
\fbox{Add hierarchical states}
\begin{definition}[\nwa] A \emph{nested word automaton} (\nwa for short) is a tuple $A=(Q, Q_0, Q_f, \Sigma, \Delta)$ where :
\begin{itemize}
\item $Q$ is the finite set of states and $Q_0, Q_f\subseteq Q$ are respectively the \emph{initial} and \emph{final} states
\item $\Delta=(\Delta_c, \Delta_r, \Delta_\text{int})$ are the set of transitions : 
\begin{itemize}
\item $\Delta_c, \Delta_\text{int}\subseteq Q\times\Sigma\times Q$ are respectively the set of \emph{call} and \emph{internal} transitions
\item $\Delta_r\subseteq Q\times Q\times\Sigma\times Q$ is the set of \emph{return} transitions
\end{itemize}
\end{itemize}
\end{definition}


\begin{remark}
Different from classical definition, no hierarchical state, but equivalent. Easing the writing of runs.
\end{remark}

\begin{definition}[run NWA] Let $w=(a_1\dots a_n, \cpl)\in \nw(\Sigma)$ and $A$ be an \nwa. The $Q$-sequence $\ell=(\ell_i)_{i\in\Ientff{0}{n}}$ is a \emph{run} of $A$ on $w$ iff : $\forall i\in[n]$, formula $\text{run}^A_i(w, \ell)$ is satisfied, where:
$$\text{run}^A_i(w, \ell)=\bigvee
\left\{
\begin{array}{l}
i\in [n]_c          \land (\ell_{i-1}, a_i, \ell_i)                                      \in \Delta_c\\%{}\\
i\in [n]_r          \land (\ell_{i-1}, q_{m^{-1}_{\cpl}(i)}, a_i, \ell_i)                \in \Delta_r\\%{}\\
i\in [n]_\text{int} \land (\ell_{i-1}, a_i, \ell_i)                                      \in \Delta_\text{int}
\end{array}
\right.$$
A run $(\ell_i)_{i\in\Ientff{0}{n}}$ is \emph{accepting} if $\ell_0\in Q_0$ and $\ell_n\in Q_f$.\\
\end{definition}

The \emph{language} recognized by $A$, denoted $L(A)$, is the set of all nested words with an accepting run on $A$. A language $L\in \nwl(\Sigma)$ is \emph{regular} if it can be recognized by an \nwa.

\begin{definition}[deterministic NWA] The \nwa $A$ is deterministic if it has a single initial state, and:
\begin{itemize}
\item $\Delta_c$ and $\Delta_\text{int}$ induce partial function from $Q\times\Sigma$ to $Q$,
\item $\Delta_r$ induces a partial function from $Q\times Q\times\Sigma$ to $Q$.
\end{itemize}
\end{definition}

\paragraph*{Determinization of \nwa}

\fbox{TBD}

==> preuve_lemme.tex <==
% !TEX root = main.tex

\begin{lemma} Let $(\ell_i)_{i\in \interv{0,n}}$ be a run of $A$ on $\omega$.  For all $0\leq k \leq n$, $\exists \overline{r} \in\overline{\mathcal{R}},  \underline{r} \in \underline{\mathcal{R}}$ such that  $( \overline{r}, \underline{r} ,\ell_k) \in L_k$.
\end{lemma}
%
%
%
%\begin{proposition} Let $0\leq k \leq n$.  If there exists $\ell$ such that $q_0 \exe{A,\interv{1,k}}{w, I} q$,  for $q_0\in Q_0$, then there exists $L$ such that  $S \exe{A,\interv{1,k}}{w, L} S'$ and $L_0=q_0'$. 
%\end{proposition}
\begin{proof}
We define: 
$$\begin{array}{rcl}
     \overline{R}: \Ientff{s-1}{f} & \to     & \overline{\mathcal{R}}^1 \cup \overline{\mathcal{R}}^2 \\
                                 i & \mapsto & \left\{\begin{array}{ll}
                                                        \overline{r} & \text{if} \ s_{\cpli}(i) < s \\ 
                                                        \ell_{s_{\cpli}(i)} &\text{if}\ s_{\cpli}(i)\in \Ientff{s}{f}^c_c\\
                                                        \ell_{s^c_c(i)} \ell_{m^{-1}_{\cplii}(s_{\cpli}(i))} \ell_{s_{\cpli}(i)} & \text{if}\ s_{\cpli}(i)\in \Ientff{s}{f}^c_r\\
                                                      \end{array}\right.\\
{}                                 & {}       & {}\\
     \underline{R}: \Ientff{s-1}{f} & \to     & \underline{\mathcal{R}} \\
                                  i & \mapsto & \left\{\begin{array}{ll}
                                                         \underline{r} & \text{if} \ s_{\cplii}(i)< s \\ 
                                                         \ell_{s_{\cplii}(i)} &\text{if}\ s_{\cplii}(i)\in\Ientff{s}{f}^2_c\\
                                                       \end{array}\right.
  \end{array}$$
\begin{remark} if $(i_1, i_2, i_3, i_4)$ is a 2 wave within $\Ientff{s}{f}$ then $\overline{R}(i_2)\preceq\overline{R}(i_3-1)$ :
\begin{itemize}
\item if $s_{\cpli}(i_2)=s_{\cpli}(i_3-1)$ e.g. $i_2$ and $i_3-1$ are covered by the same $\cpli$-arch then $\overline{R}(i_2)=\overline{R}(i_3-1)$
\item if $s_{\cpli}(i_2)<s_{\cpli}(i_3-1)$ then $s_{\cpli}(i_2) = s^c_c(i_3-1)$ e.g. $i_2$ and $i_3-1$ are covered by the same wave (but not the same arch) then :
$$\overline{R}(i_2) = \ell_{s_{\cpli}(i_2)} = \ell_{s^c_c(i_3-1)}\preceq\ell_{s^c_c(i_3-1)} \ell_{m^{-1}_{\cplii}(s_{\cpli}(i_3-1))} \ell_{s_{\cpli}(i_3-1)}=\overline{R}(i_3-1)$$
\end{itemize}
\end{remark}



We prove by induction over $k$ that $(H_{k})$:   $\forall  0 \leq i \leq k$, 
$(R_1(j),\underline{R}(j), \ell_j)\in L_j$. 
For $k=0$,  $L_0=q_0'$ and $(H_0)$ holds. Suppose $k\geq 1$,  and $( \underline{R}(i), \underline{R}(i), \ell_{i})\in L_{i}$, for all $0\leq i\leq k-1$. 

we consider the following cases: 

\begin{itemize}
\item if $k$ is an internal position then from construction of $\delta_{\text{int}}$ and  $(H_{k-1})$:  $L_k$ contains 
$(\overline{R}(k-1),\underline{R}(k-1),\ell_k)$. 
 In addition, $\overline{R}(k)= \overline{R}(k-1)$ and $\underline{R}(k)= \underline{R}(k-1)$. 

\item if $k$ is a call-call from then construction of $\delta^c_c$ and  $(H_{k-1})$,  $(\ell_k, \ell_k, \ell_k)\in L_k$. 
 In addition, $s_{\cpli}(k)=s_{\cpli}(k-1)$ hence $\overline{R}(k) = \overline{R}(k-1)$ and similarly : $\underline{R}(k)=\underline{R}(k-1)$.

 \item if $k \in [n]^r_c$, then $k=i_2$ in a wave $(i_1,i_2,i_3,i_4)$.  Since $\ell$ is a run and 
$(H_{k-1})$ holds, $(\ell_{k-1}, \ell_{i_1}, a_k,\ell_k)\in \trans{r}{c}$,  and 
\begin{equation}
\label{eq1}
(\ell_{i_1-1},a_{i_1},\ell_{i}) \in \trans{c}{c}, \ 
(\overline{R}(i_{1}-1),\underline{R}(i_1-1),\ell_{i_1-1}) \in L_{i_1-1}, \ (\ell_{i_1},\ell_{i_1},\ell_{i_1})\in L_{i_1} 
 \end{equation}
 
 From construction of $\delta_{r,c}$, $L_k$ contains 
$(\overline{R}(i_1-1), \ell_k, \ell_k)$. 
 In addition, $s_{\cpli}(k)=s_{\cpli}(i_1-1)$ hence $\overline{R}(k)=\overline{R}(i_1-1)$ and $s_{\cplii}(k)=k$ hence $\underline{R}(k)=\ell_{k}$.
 
 %%%%%%%%%%%%%
 
\item if $k \in [n]^c_r$, then $k=i_3$ in a wave $(i_1,i_2,i_3,i_4)$. Since $\ell$ is a run and 
$(H_{k-1})$ holds, $(\ell_{k-1}, \ell_{i_2}, a_k,\ell_k)\in  \trans{c}{r}$, (\ref{eq1}), and 
\begin{equation}
\label{eq2}
(\ell_{i_2-1}, \ell_{i_1} ,a_{i_2},\ell_{i_2}) \in  \trans{r}{c}, \ 
( \overline{R}(i_2), \underline{R}(i_2-1), \ell_{i_2-1})\in L_{i_2-1}, \ ( \overline{R}(i_2), \underline{R}(i_2),\ell_{i_2})\in L_{i_2} 
 \end{equation}

From construction of $ \trans{c}{r}$, 
$(\ell_k, \underline{R}(i_2-1), \ell_k) \in L_k$. 
 In addition, $s_{\cpli}(i_3)=i_3$ hence $\overline{R}(i_3)=\ell_{i_1}\ell_{i_2}\ell_{i_3}$ and $s_{\cplii}(i_3)=s_{\cplii}(i_2-1)$ hence $\underline{R}(i_3)=\underline{R}(i_2-1)$

%%%%%%%%%%%%%%%%%

\item if $k \in [n]^r_r$, then $k=i_4$ in a wave $(i_1,i_2,i_3,i_4)$. Since $\ell$ is a run and 
$(H_{k-1})$ holds, $(\ell_{k-1}, \ell_{i_3},\ell{i_1}n a_k,\ell_k)\in \trans{r}{r}$,  $(\ell_k, \ell_k, \ell_{k-1})\in L_{k-1}$, (\ref{eq1}), (\ref{eq2}) and 
\begin{equation*}
\label{eq2}
(\ell_{i_3-1}, \ell_{i_2}, a_{i_3},\ell_{i_3}) \in \trans{r}{c}, \ 
(R_1(i_1-1), \ell_k, \ell_{i_3-1}) \in L_{i_3-1}, \ ( \ell_k, \overline{R}(i_2-1), \ell_k)\in L_{i_3} 
 \end{equation*}

From construction of $\delta_{r,r}$, 
$(R_1(i_1-1), \underline{R}(i_1-1), \ell_k) \in L_{k}$. 
 In addition, $s_{\cpli}(i_4)=s_{\cpli}(i_3-1)$ hence $\overline{R}(i_4)=\overline{R}(i_3-1)$ and $s_{\cplii}(i_4)=s_{\cplii}(i_1-1)$ hence $\underline{R}(i_4)=\underline{R}(i_1-1)$.

\end{itemize}



\end{proof}


